CoPriv: Network/Protocol Co-Optimization for Communication-Efficient Private Inference

Deep neural network (DNN) inference based on secure 2-party computation (2PC) can offer cryptographically-secure privacy protection but suffers from orders of magnitude latency overhead due to enormous communication. Previous works heavily rely on a proxy metric of ReLU counts to approximate the communication overhead and focus on reducing the ReLUs to improve the communication efficiency. However, we observe these works achieve limited communication reduction for state-of-the-art (SOTA) 2PC protocols due to the ignorance of other linear and non-linear operations, which now contribute to the majority of communication. In this work, we present CoPriv, a framework that jointly optimizes the 2PC inference protocol and the DNN architecture. CoPriv features a new 2PC protocol for convolution based on Winograd transformation and develops DNN-aware optimization to significantly reduce the inference communication. CoPriv further develops a 2PC-aware network optimization algorithm that is compatible with the proposed protocol and simultaneously reduces the communication for all the linear and non-linear operations. We compare CoPriv with the SOTA 2PC protocol, CrypTFlow2, and demonstrate 2.1x communication reduction for both ResNet-18 and ResNet-32 on CIFAR-100. We also compare CoPriv with SOTA network optimization methods, including SNL, MetaPruning, etc. CoPriv achieves 9.98x and 3.88x online and total communication reduction with a higher accuracy compare to SNL, respectively. CoPriv also achieves 3.87x online communication reduction with more than 3% higher accuracy compared to MetaPruning.

==> docs/rebuttal.tex <==
\section*{Rebuttal}

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{figs/num_mul.pdf}
    % \caption{Comparison of the number of between original MobileNetV2 and CoPriv with Winograd transformation.}
    
    Figure 1: Comparison of the number of multiplications in each block between original MobileNetV2 and CoPriv with Winograd transformation (ReLU budget is set to 40\% in this example).
    
    \label{fig:enter-label}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{figs/L_comm.pdf}
    % \caption{The influence of $\mathcal{L}_{comm}$ during the search process. The bars above the x-axis means ReLU remained in this block while the bars below the x-axis means ReLU removal in this block.}
    
    Figure 2: Comparison of different pruning method and the influence of $\mathcal{L}_{comm}$ during the search in each block (ReLU budget is set to 60\% in this example).
    
    \label{fig:enter-label}
\end{figure}



\begin{table}[!h]
    \centering
    
    Table 1: Accuracy and communication comparison between refferred paper and our CoPriv.
    
    \scalebox{0.9}{
    \begin{tabular}{c|cccc}
    \hline
    Method   &  Top-1 Acc. (\%) & Online Comm. (GB) & Total Comm. (GB) \\
    \hline
    CVPRW 2023 & 69.10 & 0.81 & 46.5 \\
    CoPriv (ours)  & 70.58 & 0.43 & 5.14  \\
    \hline
    \end{tabular}
    }
\end{table}


\begin{table}[!h]
    \centering
    
    Table 2: Comparison with prior-art methods with qualitative optimization level (we take CrypTFlow2+ResNet32 on CIFAR-100 as our basline).

    % \begin{threeparttable}
    \scalebox{0.7}{
    \begin{tabular}{c|ccccrrc}
    \hline
    \multirow{2}{*}{Method} & \multirow{2}{*}{Protocol Opt.}
      & \multicolumn{3}{c}{Network Opt.}   & \multirow{2}{*}{Online Improv.}  & \multirow{2}{*}{Total Improv.}  &  \multirow{2}{*}{Example}  \\
          &             & Conv.        & Trunc.        &  ReLU       \\
    \hline
   $[33, 32, 30, 6, 29]$    &  \checkmark   &  \ding{55}   & \ding{55}     &  \ding{55}  &  - &  - & CrypTFlow2   \\
   $[25, 5, 16, 31, 28, 4]$     &   \ding{55}  &   \ding{55} &  \ding{55}    &  \checkmark  & 1.1$\sim$1.5$\times$   &  $\sim$1$\times$ &  SENet, SNL    \\
   $[27]$  & \ding{55} & \checkmark & \checkmark & \checkmark & 1.4$\sim$2.5$\times$ & 1.4$\sim$2.5$\times$ &  MetaPruning \\
     % \cite{srinivasan2019delphi,hussain2021coinn}       &   \checkmark & \ding{55}  &  \ding{55} & \checkmark  &  $\sim$3$\times$ & $\sim$4$\times$ & COINN \cite{hussain2021coinn}    \\
     $[14]$ & \checkmark & \checkmark & \ding{55} & \ding{55} & $\sim$1$\times$ & $\sim$2$\times$ &  $[14]$  \\
     \hdashline
    \method~(ours)     &    \checkmark    &      \checkmark    &   \checkmark     &   \checkmark & 2$\sim$10$\times$  & 2$\sim$4$\times$ &  Ours \\
    \hline
    \end{tabular}
    }
    % \begin{tablenotes}
    %     \scriptsize
    %     \item[*] COINN quantizes neural networks with low bitwidths to improve the efficiency.
    % \end{tablenotes}
    % \end{threeparttable}
\end{table}


% \begin{table}[!h]
%     \centering
    
%     Table 3: More ablation study of our proposed optimizations w/ KD in \method.
    
%     \label{tab:win}
%     \scalebox{0.9}{
%     \begin{tabular}{c|ccc}
%     \hline
%     Model     &  Top-1 Acc. (\%) & Online Comm. (GB) & Total Comm. (GB) \\
%     \hline
%     Baseline MobileNetV2    & 69.68  & 0.822  &  8.004 \\
%     MobileNetV2+Pruning     & 70.58  & 0.638  & 7.806 \\
%     +Re-parameterization    & 70.58  & 0.431  & 5.621  \\
%     +Winograd (\method)     & 70.58  & 0.431  & 5.144  \\
%     \hline
%     \end{tabular}
%     }
% \end{table}

\begin{table}[!h]
    \centering

     Table 3: Latency (s) comparison with Cheetah for different blocks (expand ratio is 6) and bandwidths.

    \scalebox{0.9}{
    \begin{tabular}{cccc}
    \hline
    Bandwidth                    & 384 MBps &  44 MBps  &  9 MBps     \\
    \hline
    & Dimension: $(4\times4\times64)$ \\
    \hline
    Baseline OT (CrypTFlow2)  & 2.14     &  3.55    &  16.2 \\
    HE (Cheetah)                   & 1.35     &  1.54    &  2.99\\
    CoPriv (ours)             & 0.21     &  0.64    &  3.00  \\
    \hline
    & Dimension: $(8\times8\times32)$ \\
    \hline
    Baseline OT (CrypTFlow2)  &  1.29   &  3.94  & 16.1 \\
    HE (Cheetah)                   &  0.72   &  0.73  & 1.53 \\
    CoPriv w/ Winograd (ours)       &  0.17   &  0.45   & 2.16  \\
    \hline
    \end{tabular}
    }
\end{table}

